Continual Reinforcement Learning with TELLA

Training reinforcement learning agents that continually learn across multiple environments is a challenging problem. This is made more difficult by a lack of reproducible experiments and standard metrics for comparing different continual learning approaches. To address this, we present TELLA, a tool for the Test and Evaluation of Lifelong Learning Agents. TELLA provides specified, reproducible curricula to lifelong learning agents while logging detailed data for evaluation and standardized analysis. Researchers can define and share their own curricula over various learning environments or run against a curriculum created under the DARPA Lifelong Learning Machines (L2M) Program.

==> L2M_Evaluation.tex <==
\section{L2M Evaluation}

\subsection{MiniGrid}

The most recent L2M evaluation leveraged the Minimalistic Gridworld Environment (MiniGrid) as a common environment among four performers and a baseline agent. Chosen for its simplicity, light weight, and speed, MiniGrid consists of a set of procedurally-generated environments that support a variety of actions, skills, and objectives. Another benefit of MiniGrid is its customizability with the use of wrappers to modify action space, observation space, and reward functions.

At a high level, the structure of MiniGrid environments is an NxM grid of tiles. Each tile contains either zero or one object, represented by a type, color, and state. Current provided objects include wall, floor, lava, door, key, ball, box, and goal, each having their own properties depending on the environment (e.g., can be picked up, can be dropped, or can be toggled). There are seven available actions that the agent can take each time step: turn left, turn right, move forward, pick up an object, drop the object being carried, toggle object, and done (task completed). The default reward function is sparse, returning a -1 for colliding with obstacles, zero for failure to complete the objective in a specified time step limit, and a positive reward of 1 minus a time step penalty on success. 

In order to exercise lifelong learning and adaptation to new tasks, six MiniGrid tasks were chosen for the experimentation with three variants each: 

\begin{itemize}
    \item \textbf{Simple Crossing}: Agent navigates through simple maze to reach goal. Parameters for variation include grid size and number of crossings.
    \item \textbf{Distributional Shift}: Agent navigates to goal while avoiding lava. Parameters for variation include location of lava strip.
    \item \textbf{Dynamic Obstacles}: Agent navigates to goal while avoiding moving obstacles. Parameters for variation include grid size and number of obstacles.
    \item \textbf{Custom Fetch}: Agent must pick up a yellow key. This differs from the provided Fetch environment because in that environment, the target object is randomly generated and identified with a mission string. Parameters for variation include grid size, number of targets, and number of objects.
    \item \textbf{Unlock}: Agent must pick up a key to unlock a door. Parameters for variation include room size.
    \item \textbf{Door and Key}: Agent navigates to goal after unlocking a door with a key. Parameters for variation include grid size.
\end{itemize}

\subsection{L2M Curricula}

Two unique types of curricula (shown in Figure \ref{fig:curriculum_diag}) were designed for the L2M evaluation with 100 runs per curriculum, where each run represents a different random permutation of task variant training order.

\textbf{Condensed}: The Condensed curriculum is an interleaving sequence of evaluation and training blocks, where each task variant is trained exactly once and all task variants are evaluated in each evaluation block.
 
\textbf{Dispersed}: The Dispersed curriculum is an interleaving sequence of evaluation and training blocks, where each task variant is trained three times and all task variants are evaluated in each evaluation block. There are three "superblocks" which make up the dispersed curriculum, where a superblock is defined as a single permutation of task variants with short learning blocks (1/3 the length of the condensed learning blocks). A given task variant occurs exactly once during each superblock and each superblock uses a different random permutation of task variants.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{minigrid_environments.png}
    \caption{MiniGrid Environments}
    \label{fig:minigrid_environments}
\end{figure}

\subsection{Evaluation Metrics}

By integrating with L2Logger and L2Metrics, \tella enables the use of seven different metrics to evaluate the performance of agents in RL and supervised learning contexts.

% Refer to lifelong learning metrics specification

\textbf{Performance Maintenance (PM)}: Performance maintenance measures how much an agent catastrophically forgets a previously-learned task. This metric is calculated by taking the average difference between task evaluation performance and the evaluation performance immediately following the task's most recent training block, throughout a lifetime.

\textbf{Mean Training Performance (MTP)}: Mean training performance measures how much an agent has learned a task during training. This metric is calculated by taking the arithmetic mean of task performance across a lifetime, essentially a normalized area under the curve.

\textbf{Mean Evaluation Performance (MEP)}: Mean evaluation performance measures how much performance an agent retains as it learns more tasks throughout a lifetime. This metric is calculated by taking the arithmetic mean of task evaluation performance.

\textbf{Forward Transfer (FT)}: Forward transfer measures how much an agent improves learning on a new task by leveraging experience from previously-learned tasks. Existing literature often calls this a "jumpstart" formulation of the concept of forward transfer, which measures the boost in performance one task gives to another when the second task is first seen.

\textbf{Backward Transfer (BT)}: Backward transfer measures how much an agent improves learning on a previously-learned task by leveraging experience from a new task. This is a "jumpstart" formulation of the concept of backward transfer, which measures the boost in performance one task gives another when the second task is first seen.

\textbf{Relative Performance (RP)}: Performance relative to a Single-Task Expert measures how well a lifelong learning system is doing compared to a non-lifelong learner with comparable learning experience. This metric is calculated by taking the ratio of area under performance curves for the same amount of training experience.

\textbf{Sample Efficiency (SE)}: Sample efficiency measures how quickly and efficiently an agent learns over the course of its lifetime compared to a Single-Task Expert. This metric is a composite of two ratios involving saturation values and experience to saturation.

\subsection{Evaluation Results}

The L2M evaluation resulted in a successful cross-algorithm comparison with a non-lifelong learning baseline agent. The use of \tella and MiniGrid allowed for a sufficient number of runs for statistically reliable results, enabling deeper insight into agent performance. The common set of tasks and baselines also revealed limitations in evaluation metrics, leading to alternative metrics and an improved analysis approach for the future.

Figure \ref{fig:l2m_results} shows the final results of the evaluation, where the green shaded regions represent a lifelong learning threshold for each respective metric. The right-most bar plot in each graph is the non-lifelong learning baseline and it can be seen that, on average, the performers are exhibiting greater lifelong learning capabilities than the baseline.

\cash{Have we cleared this figure with Gautam? We talk about this as a final result of the evaluation and the results don't look too good for the performers compared to the baseline. Can we refer to this as an evaluation of 4 different algorithms and not say that it came from the official L2M results?}

\eric{This figure is mostly a placeholder and has not been cleared by Gautam. There is a more updated plot I can throw in here that actually uses the seven metrics defined above. I'm okay with referring to lifelong learning algorithms as opposed to performers.}

% TODO: Update plot with new results showing clearer trend
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth, height=10cm, keepaspectratio]{l2m_results.png}
    \caption{L2M Results}
    \label{fig:l2m_results}
\end{figure*}
\label{m21}

